Exploring the Limits of Natural Language Inference Based Setup for Few-Shot Intent Detection

Intent Detection is one of the core tasks of dialog systems. Few-shot Intent Detection is challenging due to limited number of annotated utterances for novel classes. Generalized Few-shot intent detection is more realistic but challenging setup which aims to discriminate the joint label space of both novel intents which have few examples each and existing intents consisting of enough labeled data. Large label spaces and fewer number of shots increase the complexity of the task. In this work, we employ a simple and effective method based on Natural Language Inference that leverages the semantics in the class-label names to learn and predict the novel classes. Our method achieves state-of-the-art results on 1-shot and 5-shot intent detection task with gains ranging from 2-8\% points in F1 score on four benchmark datasets. Our method also outperforms existing approaches on a more practical setting of generalized few-shot intent detection with gains up to 20% F1 score. We show that the suggested approach performs well across single and multi domain datasets with the number of class labels from as few as 7 to as high as 150.

==> IEEEtran/tools/README <==

January 11, 2007


The IEEEtrantools.sty package provides several commands from the
IEEEtran.cls file so that they can be used under other LaTeX classes. The
user guide provided here covers only the differences in the use of the
commands from those provided by IEEEtran.cls. For complete documentation
on these commands, see the relevant sections in the IEEEtran_HOWTO manual
of the IEEEtran LaTeX class.

The IEEEtrantools.sty package provides the following IEEEtran.cls commands:

 1. \IEEEPARstart which produces large initial "drop cap" letters.
 2. the \bstctlcite command for the control entry types of IEEEtran.bst
    V1.00 and later
 3. the IEEE itemize, enumerate and description list environments
 4. the complete IEEEeqnarray family for producing multiline equations
    as well as matrices and tables, including the IEEEeqnarray support
    commands.

IEEEtrantools.sty should not be used with IEEEtran.cls.

For helpful tips, answers to frequently asked questions and other support,
visit the IEEEtrantools support page at my website:

http://www.michaelshell.org/tex/ieeetran/tools/


Enjoy!

Michael Shell
http://www.michaelshell.org/


*******
1/2007 V1.2 (V1.7 of IEEEtran.cls) changes:

 1. Several commands and enviroments have depreciated in favor of
    replacements with IEEE prefixes to better avoid potential future name
    clashes with other packages. Legacy code retained to allow use of the
    obsolete forms, but with an warning message to the console during
    compilation:
    \IEEEPARstart
    For IED lists:
    \IEEEiedlabeljustifyc, \IEEEiedlabeljustifyl, \IEEEiedlabeljustifyr,
    \IEEEnocalcleftmargin, \IEEElabelindent, \IEEEsetlabelwidth,
    \IEEEusemathlabelsep
 
 2. These commands/lengths now require the IEEE prefix and do not have
    legacy support: \IEEEnormaljot.
    For IED lists: \ifIEEEnocalcleftmargin, \ifIEEEnolabelindentfactor,
    \IEEEiedlistdecl, \IEEElabelindentfactor

 3. \normalsizebaselineskip no longer provided. 

 4. New \IEEEPARstart controls:
    \IEEEPARstartHEIGHTTEXT, \IEEEPARstartFONTSTYLE, \IEEEPARstartCAPSTYLE,
    \IEEEPARstartWORDFONTSTYLE, \IEEEPARstartWORDCAPSTYLE,
    \IEEEPARstartHOFFSET, \IEEEPARstartITLCORRECT
    and the (output) length \IEEEPARstartletwidth.

 5. Provide for an optional argument to \bstctlcite to provide a way to
    specify a different aux file. Define \bstctlcite even if it has already
    been defined.

********************************** Files **********************************

README                - This file.

IEEEtrantools.sty     - The LaTeX package file.

IEEEtrantools_doc.txt - The user manual - supplementary to the 
                        IEEEtran_HOWTO manual.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtrantools.sty, IEEEtrantools_doc.txt
***************************************************************************



==> related.tex <==
\section{Related Work}
% In Few-shot learning the classifiers are required to generalize to unseen (or novel) classes with only a few training examples per class (called the support set). Transfer learning and meta-learning are two conventional techniques that have been applied to address the challenge of data scarcity. The paradigm of transfer learning usually refers to pre-training initial models using mismatched domains with rich human annotations and then adapting the models with limited labels in targeted domains. Meta learning is the paradigm of learning to learn, and it intends to design models that can learn new skills or adapt to new environments rapidly with a few training examples.

% Previous works \cite{yang2017transfer, chen2019bert} have shown promising results in applying transfer learning to FSL tasks. Meta-learning has gained growing interest among the machine learning fields for tackling the problems in few-shot learning and data scarcity.
Previous works adopt metric-based approaches like prototypical networks (ProtoNets) \cite{DBLP:conf/nips/SnellSZ17} and matching networks \cite{vinyals2016matching} for the task of few-shot learning. \citet{DBLP:conf/nips/SnellSZ17} represents the class prototypes by support samples and uses euclidean distance to infer the class of a new data sample. With matching networks \citet{vinyals2016matching} aim to learn an embedding space which can be generalized to domains new to the training set after adaptation with a small number of examples from the novel domains. Another type of meta learning approach called Model-Agnostic Meta-Learning (MAML) \cite{finn2017model} focuses on learning parameter initialization from multiple subtasks, such that the initialization can be fine-tuned with few labels
yielding good performance in targeted tasks. Compared to metric based approaches, optimization based approaches generally perform poorly on intent detection task \cite{DBLP:conf/slt/0001KDZA21}. Therefore, in this work we focus our comparison with metric-based approaches. 


Recently, many FSL works which make use of multi-level matching and aggregation methods to improve FSL performance \cite{gao2019hybrid} have been proposed. The basic idea is to integrate matching information between support and query samples on multiple levels. \citet{nguyen-etal-2020-dynamic} extracts multiple semantic components from support and query sentences via multi-head self-attention with additional regularizations. \citet{ye-ling-2019-multi} builds local context representation for both support and query samples using a soft matching approach. \citet{sun2019hierarchical} added word-level attention and uses a more advanced multi-cross attention upon instance level. Although these approaches have shown promising results in few-shot intent detection, there is still considerable room for improvement as shown in our comparisons.

Textual entailment has been explored in previous works as a promising approach for few-shot text classification. \citet{DBLP:journals/corr/abs-2104-14690} focuses on a common benchmarks of single sentence and sentence pair few-shot classification tasks using a BERT model fine-tuned upon MNLI dataset. 
% \citet{ma2021issues} solely focuses upon disadvantages of zero shot text classification using entailment based few-shot learning.
\citet{sainz-etal-2021-label} attempts to utilize NLI based few-shot learning for Relation Extraction. For the task of intent detection \citet{zhang-etal-2020-discriminative} focuses upon the detection of out-of-scope intents. In general, primary motivation of the previous works was to measure the generalizability of the NLI based few-shot learning for different NLP tasks. Our work focuses upon the application of the NLI based few-shot learning setup for intent detection and we compare this approach with several competitive baselines. To the best of our knowledge, we are the first to conduct extensive experiments that shed light on the experimental settings where the NLI based method is extremely effective for few-shot intent detection.

